H-NeXt: The next step towards roto-translation invariant networks

The widespread popularity of equivariant networks underscores the significance of parameter efficient models and effective use of training data. At a time when robustness to unseen deformations is becoming increasingly important, we present H-NeXt, which bridges the gap between equivariance and invariance. H-NeXt is a parameter-efficient roto-translation invariant network that is trained without a single augmented image in the training set. Our network comprises three components: an equivariant backbone for learning roto-translation independent features, an invariant pooling layer for discarding roto-translation information, and a classification layer. H-NeXt outperforms the state of the art in classification on unaugmented training sets and augmented test sets of MNIST and CIFAR-10.

==> tables/cifar-rot-test.tex <==
% Fix degrees UTF-8 \circ
\begin{tabular}{lrrrr}
\hline
                   Model                   &  Test        & Val. $45^\circ$  & Val.  & \# params \\
\hline\hline
\textbf{UP}+\textbf{MASK}                &  56.41 ± 0.82 &  55.27 ± 0.80 &  60.22 ± 0.99 & 28k \\
\textbf{UP}+\textbf{MASK}+\textbf{HUGE}  &  58.75 ± 1.23 &  57.68 ± 0.28 &  65.35 ± 0.73 & 398k  \\
\textbf{UP}+\textbf{MASK}+\textbf{WIDE}&  59.50 ± 1.33 &  58.10 ± 1.42 &  63.22 ± 1.11 & 100k  \\
\textbf{UP}+\textbf{MASK}+\textbf{MSA} &  59.95 ± 0.61 &  57.46 ± 0.46 &  64.53 ± 0.32 & 118k  \\

\hline
\end{tabular}


==> tables/mnist-rot-test.tex <==
\begin{tabular}{lrrr}
\hline
                   Model    &  Test     & Val. $45^\circ$  & Val. \\
\hline\hline
\ac{hnet}    &     92.9 $\pm$ 1.02 & 84.8  $\pm$ 1.68    &    98.5 $\pm$ 1.51 \\
\textbf{UP}  &     95.9 $\pm$ 0.62 & 91.6 $\pm$ 0.83  &  98.9 $\pm$ 0.06 \\
\textbf{UP}+\textbf{MASK} &     98.7 $\pm$ 0.11 & 97.8  $\pm$ 0.20   &  98.9 $\pm$ 0.08 \\

\hline
\end{tabular}


==> tables/rotated-mnist.tex <==
\begin{tabular}{lrl}
\hline
Model                             & Test Error   & \# Param.  \\
\hline\hline
SVM (RBF) \cite{larochelle2007} &10.38 $\pm$ .1500  & -  \\
CNN  \cite{cohen2016}       &5.03 $\pm$ .0004 &          22k \\
CNN (with data aug) \cite{cohen2016}       &3.50 $\pm$ .0004 &          22k \\
 (rot. pool) \cite{cohen2016}       &2.28 $\pm$ .0004 &          25k \\
p4CNN  \cite{cohen2016}       &2.28 $\pm$ .0004 &          25k \\
\ac{hnet}  \cite{worrall2017}     &1.69 $\pm$ .???? &          33k \\
CFNet  \cite{chidester2019}       &1.75 $\pm$ .???? &          - \\
PDO-eConv  \cite{shen2020}       &1.87 $\pm$ .???? &          26k \\
\textbf{E(2)-CNN} ($D_{16}\mid_{5}C_{16}$) \cite{weiler2018}       & \textbf{.682 $\pm$ .0220} &          26k \\
PDO-eConv + PCETs \cite{singh2022a}     &1.56 $\pm$ .0004 &   27.5k \\
\ac{hnext} & $1.50  \pm .1130  $& 25.3k \\
\hline
\end{tabular}
